Linear Hybrid System Falsification With Descent

In this paper, we address the problem of local search for the falsification of hybrid automata with affine dynamics. Namely, if we are given a sequence of locations and a maximum simulation time, we return the trajectory that comes the closest to the unsafe set. In order to solve this problem, we formulate it as a differentiable optimization problem which we solve using Sequential Quadratic Programming. The purpose of developing such a local search method is to combine it with high level stochastic optimization algorithms in order to falsify hybrid systems with complex discrete dynamics and high dimensional continuous spaces. Experimental results indicate that indeed the local search procedure improves upon the results of pure stochastic optimization algorithms.

==> hybrid_results.tex <==
\subsection{Numerical experiments}\label{subsecHybRes}

To illustrate the usage of the Robustness Ellipsoid Descent (RED) approach, we run three experiments: first, we simply choose five different initial points, and solve Program \ref{eqHybridProg} at each initial point, and report the results. Next, we run the Monte-Carlo Falsification (MCF) method of \cite{JuliusFALP07hscc} 5 different times. Each time, MCF will return the least robust initial point it found. We use this as input to our method, and show that it is able to find even less robust trajectories around it. Finally, we integrate RED in MCF: at each initial point proposed by MCF, we run RED to optimize the robustness locally. Then, control is handed back to MCF to propose a new starting point at which to run the local optimization, and so on.

We implemented our techniques in MATLAB$^{TM}$. We used the built-in function fmincon with algorithm `SQP'. We halt the optimization as soon as the objective function value is less than $0$ (meaning that all constraints are satisfied). This also helps reduce the run-time.

For the second experiment, we present three illustrative sample results: on three different runs, MCF returned three points with (truncated) robustness values of 0.105566, 0.107499 and 0.14704. Running RED from these initial points, it found three trajectories with robustness values of, respectively, 0.105472, 0.105486 and 0.10378. Thus RED succeeded in improving the results of MCF. 

Experimentally, we noted a fast convergence of RED to local minima: a few iterations were typically sufficient to stop improvement of the objective function, and of the robustness.

For 




==> jointOptGlobalMin.tex <==
\subsection{Correspondance of global minima}\label{sec:jointOptGlobalMin}

	Finally, we show that should Algorithm \ref{alg:red} reach a global minimum of $F$, then it is also a global minimum of $f$. This isn't obvious from Proposition \ref{prop:localMin}: while every local minimum of $F$ maps to a local minimum of $f$, $f$ might have, \emph{a priori}, some local minima that do not correspond to any minima of $F$. Moreover, this mapping between minima is purely local, and does not allow us to compare values of different minima of $f$.
	
	We prove this result for the case where the global minimum is safe, i.e. the least robust trajectory does not enter the unsafe set (otherwise, our work is done as we have found an unsafe trajectory). We also assume that the descent set is polyhedral. The more general case (general convex) has not been studied yet.
	
	We introduce some additional notation.
	\begin{defn} [$\Xi, \Xi^+_p$]
	Given a polyhedron $\unsafe$, let $\Xi = \{H_i\}$ be the set of hyperplanes that bound it, $H_i = \{x|a_i^Tx = b_i\}$.
	For a given point $p \in \Re^n$, let $\Xi^+_p \subseteq \Xi$ be the set of hyperplanes that separate $p$ from the origin of reference $\mathbf{0}$:
	\[\Xi^+_p = \{H_i \in \Xi | a_i^Tp \geq b_i\} \]	
	\end{defn}
	
	\begin{defn}[slack]
	Given $p \in \Re^n$ and a hyperplane $H$, $slack(p, H) =a^Tp-b$ is the slack of $p$ relative to $H$. 
	\end{defn}	
	
	To prove our result, we need the following lemmata: they connect the notion of maximum slack to the notion of minimum distance, thus allowing us to infer statements about robustness (minimum distance) from statements about the objective function $F$ (smallest maximum slack). In all that follows, $p$ is an arbitrary point outside $\unsafe$, and $H$ is an arbitrary hyperplane in $\Xi$. Without loss of generality, it is assumed that the origin of reference $\mathbf{0}$ lies inside $\unsafe$, thus $b_i \geq 0$ for all $i$.
	
	
	\begin{lemma}\label{lemma:z}
	Let $\unsafe$ be a polyhedron and $p \in \partial \unsafe$. If $H \in \Xi$ is such that $p \notin H$, then $a^Tp<b$.
	\end{lemma}
	\begin{proof}
	$p \notin H$ so $a^Tp \neq b$. Assume, for contradiction, that $a^Tp > b$. Then, by continuity of $a^Tx$ in the variable $x$, $\exists B(p;\epsilon)$ s.t. $a^Tx > b$ for all $x \in B$. But $p \in \partial \unsafe \Rightarrow B \cap \unsafe \neq \emptyset$. For points in $B \cap \unsafe$, $a^Tx \leq b \Rightarrow$ contradiction.
	\end{proof}
	
	\begin{lemma}\label{lemma:0}
	\[slack(p,h \in \Xi^+_p) \geq 0\]
	\end{lemma}
	\begin{proof}
	Immediate from the definitions.
	\end{proof}
			
	\begin{lemma}\label{lemma:1}
	$|slack(p,H)| = d_H(p)$
	\end{lemma}
	\begin{proof} 
	Let $H =\{x|a^Tx = b\}$. There are three cases (See Fig. XXX ):\\
	\underline{Case 1:} $a^Tp\geq b$.\\
	 Then $d_H(p) = a^Tp-b = slack(p,H) \geq 0$\\ 
	\underline{Case 2:} $0 \leq a^Tp < b$. \\
	Then  $d_H(p) = b-a^Tp = - slack(p,H) > 0$ \\
	\underline{Case 3:} $a^Tp < 0$. \\
	Then $d_H(p) = b+|a^Tp| = b-a^Tp = - slack(p,H) > 0$ 
	\end{proof}
	
	\begin{lemma}\label{lemma:2}
	\[H' \triangleq arg\max_{h \in \Xi} slack(p,h) \in \Xi^+_p\]
	\end{lemma}
	\begin{proof}
	$\Xi^+_p$ is non-empty since it is assumed that $p$ is outside $\unsafe$, and therefore $a^Tp > b$ for at least one hyperplane $H$. By Lemma \ref{lemma:0}, $slack(p,h \in \Xi^+_p) \geq 0$, whereas $slack(p,h \in \Xi - \Xi^+_p) < 0$. Thus the maximum slack is achieved by a hyperplane in $\Xi^+_p$.
	\end{proof}
			
	
	\begin{lemma}\label{lemma:3}
	Let $u^*$ be the point of $\overline{\unsafe}$ closest to $p$, and $H^*$ a hyperplane to which $u^*$ belongs. Then
	$H^*$ is the farthest hyperplane to $p$ among the hyperplanes in $\Xi^+_p$:
	\[H^* = arg\max_{h \in \Xi^+_p} d_h(p)\]	
	\end{lemma}
	
	\begin{proof}	
	$H^* \in \Xi^+_p$. Let $h$ be another hyperplane in $\Xi^+_p$. Then
	\[d_{H^*}(p) = a^Tp-b\]
	\[d_{h}(p) = a_h^Tp-b_h\]
	But we already proved (Lemma \ref{lemma:z}) that $a_h^Tp \leq b_h + d_{H^*}(p)$\\
	$\Leftrightarrow d_{H^*}(p) \geq d_{h}(p) \forall h \in \Xi^+_p$
	\end{proof}
	
	\begin{lemma}\label{lemma:4}
	i) $H'$ contains $u^*$\\
	ii) $d_{H'}(p) = d_\unsafe(p)$
	\end{lemma}
	
	\begin{proof}
	i) By Lemmata \ref{lemma:2}\&\ref{lemma:3}
	\begin{equation*}
	\begin{split}
	H^* &= arg\max_{h \in \Xi^+_p} d_h(p)\\
	     &= arg\max_{h \in \Xi^+_p} slack(p,h) \\
				& = H'	
	\end{split}
	\end{equation*}
	Therefore $H'$ contains $u^*$. \\
	ii) Since $u^* \in H'$, $d_{H'}(p) = ||p-u^*|| = d_\unsafe(p)$.
	\end{proof}
	
	The stage is now set to state and prove our main result:
	\begin{proposition}\label{prop:globalMin}
	Let $z = (x,t,\nu)$ be a global minimum of $F$ in problem Prob\ref{eqHybridProg}[$\unsafe$]. Then $x$ is a global minimum of $f$ over $E(x_0) \bigcap X_0$. 	
	\end{proposition}
	
	\begin{proof}
	Consider $x' \in E(X_0) \bigcap X_0, x' \neq x$. 
	Let $t'$ be the time at which the trajectory $s_{x'}$ is closest to $\unsafe$, and let $p = s_{x'}(t')$ to simplify notation.
	We can now construct $z'$: 
	\[z' = (x', t', \nu') = (x', t', \max_{h \in \Xi}slack(p, h))\]
	
	Let $H'$ be the hyperplane that achieves the maximum in above expression, and $H$ be the hyperplane that achieves the maximum slack for $s_x(t)$.
	 
	Clearly, $z' \neq z$. Because $z$ is a global minimum of $F$, then
	\begin{equation*}
	\begin{split}
	& F(z') \geq F(z)\\
	\Leftrightarrow & \max_{h \in \Xi}slack(p, h)     \geq \max_{h \in \Xi}slack(s_x(t), h) \\
	\Leftrightarrow & \max_{h \in \Xi^+_p}slack(p, h) \geq \max_{h \in \Xi^+_{s_x(t)}}slack(s_x(t), h) \textrm{ (by Lemma \ref{lemma:2})} \\
	\Leftrightarrow & slack(p, H') \geq slack(s_x(t), H) \textrm{ (by def. of $H$ and $H'$)} \\
	\Leftrightarrow & d_{H'}(p) \geq dist_{H}(s_x(t)) \textrm{ (by Lemmata \ref{lemma:0}\&\ref{lemma:1})} \\
	\Leftrightarrow & d_\unsafe(p) \geq dist_\unsafe(s_x(t)) \textrm{ (by Lemma \ref{lemma:4}.ii)} \\
	\Rightarrow & d_\unsafe(s_{x'}(t')) \geq min_\tau dist_\unsafe(s_x(\tau)) = f(x) \\
	\Rightarrow & f(x') \geq f(x)  \textrm{ by def. of $t'$}\\
	\end{split}
	\end{equation*}	
	Since $x'$ was chosen arbitrarily, $x$ is a global minimum of $f$ over $E(x_0) \bigcap X_0$.	 
	\end{proof}
	


==> subsecExhaustiveDesc.tex <==
	\subsection{Exhaustive descent}\label{subsecExhaustiveDesc}
	Recall that by choosing 
	
	\[d \in (X_0 - x_0) \bigcap e^{-At^*}[P_c(x_0; t^*) - s_{x_0}(t^*)] \]
	
	the new trajectory (starting at $x_0 + d$) will achieve the new distance at the same moment $t^*$ as the original trajectory. But this is not necessary: the time at which the new distance is achieved is immaterial, so long as it is smaller than the previous robustness. So what if, instead of shifting $s_{x_0}(t^*)$ closer, we shifted another $s_{x_0}(\tau)$? 
	
	Define the set (see Fig \ref{fig:PcPc})
	$$T(t^*) = \bigcup \{\tau \geq 0 | P_c(x_0; t^*) \bigcap P_c(x_0; \tau) \neq \emptyset\}.$$ 
Then, for any $\tau \in T(t^*)$, choose $d'$ s.t.
	\begin{equation*}
	\begin{split}
	s_{x_0}(\tau) + &d' \in P_c(x_0; t^*) \bigcap P_c(x_0; \tau) \\
									&d' \in P_c(x_0; t^*) \bigcap P_c(x_0; \tau) - s_{x_0}(\tau) \\
									&d = e^{-A\tau}d' \\
			\Rightarrow & d \in (X_0 - x_0) \bigcap  e^{-A\tau} [P_c(x_0; t^*) \cap P_c(x_0; \tau)- s_{x_0}(\tau) ]
	\end{split}
	\end{equation*}
	
	As this holds for all $\tau \in T(t^*)$, it comes	
	\begin{equation}\label{eqExhaustiveDesc}
	d \in (X_0 - x_0) \bigcap \{\cup_{\tau \in T(t^*)} e^{-A\tau}[P_c(x_0; t^*) \cap P_c(x_0; \tau) - s_{x_0}(\tau)]\} 
	\end{equation}
		
This will be referred to as the `exhaustive set'.

\begin{figure}[ht]
\centering
\includegraphics[width=110pt]{fig02}
\caption{The unsafe set $\unsafe$ and the sets $P_c(x_0; t^*)$ and $P_c(x_0; \tau)$. 
The shaded area is the set $P_c(x_0; t^*) \cap P_c(x_0; \tau)$.}
\label{fig:PcPc}
\end{figure}
	
What do we gain by doing this? Since $s_{x_0}(\tau) + d' \in P_c(x_0; t^*)$, it is closer to $\unsafe$ than $s_{x_0}(t^*)$, so the exhaustive set,  Eq.(\ref{eqExhaustiveDesc}), is a descent set. And, since $t^* \in T(t^*)$, the exhaustive set is larger than the partial descent set in Eq.(\ref{eqParDescPc}). 
	
	\todo[inline]{Are there any (useful) relations between $e^{A\tau}$ and $e^{A\tau'}$?}
	
	\todo[inline]{GF: An interval based approximation of $e^{At}$ might be useful in this case}
	
